A survey on real-time 3D scene reconstruction with SLAM methods in embedded systems

The 3D reconstruction of simultaneous localization and mapping (SLAM) is an important topic in the field for transport systems such as drones, service robots and mobile AR/VR devices. Compared to a point cloud representation, the 3D reconstruction based on meshes and voxels is particularly useful for high-level functions, like obstacle avoidance or interaction with the physical environment. This article reviews the implementation of a visual-based 3D scene reconstruction pipeline on resource-constrained hardware platforms. Real-time performances, memory management and low power consumption are critical for embedded systems. A conventional SLAM pipeline from sensors to 3D reconstruction is described, including the potential use of deep learning. The implementation of advanced functions with limited resources is detailed. Recent systems propose the embedded implementation of 3D reconstruction methods with different granularities. The trade-off between required accuracy and resource consumption for real-time localization and reconstruction is one of the open research questions identified and discussed in this paper.

==> evaluation.tex <==
The performance of SLAM methods, from localization to 3D reconstruction, is based on several metrics \cite{Bodin2018, Bujanca2019} for the accuracy of the estimated trajectory (m), reconstruction (m) \cite{Whelan2015}, depth and semantic segmentation (\%). The processing times provide useful information for real-time performance of isolated functions and for the whole pipeline (s, Hz, or FPS). \par

The trajectory is mostly assessed on the precision of the absolute trajectory error (ATE) \cite{grupp2017evo, Sturm2012}. The estimated and the ground truth trajectories are matched with the $SE(3)$ or $Sim(3)$ alignment \cite{Umeyama1991} for visual-inertial and pure monocular approaches respectively. Then, the root mean square error (RMSE) is computed to provide the error metric in meters \cite{ZhangIROS2018}. The ATE RMSE quantify the quality of the entire estimated trajectory. Real-time localization methods based on relative measurements drift over time. Therefore, the relative position error (RPE) allows the evaluation of the accumulated error on trajectory segments at different time intervals of the distance traveled (in m/s) \cite{Delmerico2018}. \par

Quantitatively, the 3D reconstruction is evaluated based on the average Euclidean distance between the ground truth point cloud and the estimated one generated from the reconstructed scene \cite{Rosinol20icra-Kimera}. Both representations are registered with the ICP algorithm \cite{Besl1992, Zhou2018}. In \cite{Wang2020}, the accuracy of the estimated point cloud is assessed with the reconstruction error (RE):

\begin{equation}
    RE = \frac{1}{m}\sum_{j=0}^{m}(\frac{1}{n_{j}}\sum_{i=0}^{n_{j}}(d_{err,i,j}))
\end{equation}
where $m$ is the total number of keyframes, $n_{j}$ the total number of 3D points related to keyframe $j$ and $d_{err,i,j} = \frac{\lVert(P - \Delta*\hat{P})\rVert}{\lVert(P)\rVert}$. $P$ is the GT position of the estimated 3D point $\hat{P}$ and $\Delta$, the rigid-body transformation of features from image to real-world coordinate \cite{Sturm2012}. Qualitatively, the reconstruction is compared with various granularities. In \cite{Dai2016}, specific parts of the reconstructed scene are highlighted to demonstrate the quality of the reconstruction. In \cite{Oleynikova2016}, different voxel sizes (0.02 m to 0.20 m) are compared to show the quality of the structure at small and large voxel dimensions. \par

The accuracy of the 3D reconstruction highly depends on the depth estimation precision. The latter computes several error metrics used in the literature \cite{Eigen2014}: the percentage of accurate depths ($\delta$) within a threshold ($thr$), the average relative error (rel) between the ground truth $y_{i}$ and estimated $\hat{y}_{i}$ depths at each pixel $i$, the squared relative difference (sq\_rel), the RMSE(linear) and the RMSE($\log_{10}$):

\begin{itemize}
    \item $max(\frac{y_{i}}{\hat{y}_{i}},\frac{\hat{y}_{i}}{y_{i}}) = \delta < thr, thr \in \left\{\begin{matrix} 1.25, 1.25^2, 1.25^3 \end{matrix}\right\}$
    \item rel = $\frac{1}{N}\sum_{i=1}^{N}\frac{\left | y_{i} - \hat{y}_{i} \right |}{y_{i}}$, with $N$ the total number of depths.
    \item sq\_rel = $\frac{1}{N}\sum_{i=1}^{N}\frac{\lVert y_{i} - \hat{y}_{i} \rVert^2}{y_{i}}$
    \item RMSE(linear) = $\sqrt{\frac{1}{N}\sum_{i=1}^{N}\lVert y_{i} - \hat{y}_{i}\rVert^2}$
    \item RMSE($\log_{10}$) = $\sqrt{\frac{1}{N}\sum_{i=1}^{N}\lVert \log y_{i} - \log \hat{y}_{i}\rVert^2}$
\end{itemize}

\noindent The evaluation of intermediate representations also involves an error metric for semantic segmentation based on the intersection over union (IoU) which computes the percentage of overlap between the predicted segmentation and the ground truth for each class. \par
